Constraint-based type inference for FreezeML

FreezeML is a new approach to first-class polymorphic type inference that employs term annotations to control when and how polymorphic types are instantiated and generalised. It conservatively extends Hindley-Milner type inference and was first presented as an extension to Algorithm W. More modern type inference techniques such as HM(X) and OutsideIn($X$) employ constraints to support features such as type classes, type families, rows, and other extensions. We take the first step towards modernising FreezeML by presenting a constraint-based type inference algorithm. We introduce a new constraint language, inspired by the Pottier/R\'emy presentation of HM(X), in order to allow FreezeML type inference problems to be expressed as constraints. We present a deterministic stack machine for solving FreezeML constraints and prove its termination and correctness.

==> figures/constraint-aux.tex <==
\begin{figure}[htb]

$$
\bl
\ba[t]{@{}r@{~}c@{~}l}

\fv(\true)                       &=& \emptyset\\
\fv(A \ceq B)                       &=& \emptyset\\
\fv(C_1 \wedge C_2)           &=& \fv(C_1) \cup \fv(C_2)\\

\fv(\exists (a : R). C)             &=& \fv(C) \\
\fv(\forall a. C)             &=& \fv(C) \\

\fv(x \preceq A)              &=& \lbrace x \rbrace \\

\fv(\freeze{x : A})           &=& \lbrace x \rbrace \\

\fv(\Def\; (x : A) \;\In\; C) &=& \fv(C) \setminus \lbrace x \rbrace \\

\fv(\Let_R\; x = \letexists{a} C_1 \;\In\; C_2) &=&
\fv(C_1) \cup (\fv(C_2) \setminus \lbrace x \rbrace) \\

\ea
\el
$$

\caption{Constraints Auxiliary Definitions.}
\label{fig:contraints-aux}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/constraint-generation.tex <==
\begin{figure}[ht]

\[
\ba{@{}r@{~\;}c@{~\;}l@{}l@{}r@{}}
\congen{\freeze{x} : A}                     &=& \freeze{x : A} && \parlab{C-Freeze} \\
\congen{x : A}                              &=& x \preceq A && \parlab{C-Inst} \\
\congen{M\,N : A}                           &=&
 \exists a. (\congen{M : a \to A} \wedge \congen{N : a} )&& \parlab{C-App} \\

\congen{\lambda x.M : A}                    &=&
 \multicolumn{2}{l}{
 \exists a_1,  a_2. (a_1 \to a_2 \ceq A \wedge \Def\; (x : a_1)\; \In \;\congen{M : a_2})} & \parlab{C-Abs} \\

\congen{\lambda (x : B).M : A}              &=&
 \multicolumn{2}{l}{
 \exists a_1. B \to a_1 \ceq A \wedge \Def\; (x: B) \;\In\; \congen{N : a_1}} & \parlab{C-AbsAscribe} \\

\congen{\Let \; x = U\; \In \; N : A}       &=&
  \Let\phantom{_\mono} \; x = \letexists{a} \congen{U : a} \; \In \;\congen{N : A} && \parlab{C-LetVal} \\

\congen{\Let \; x = M\; \In \; N : A}       &=&
 \Let_\mono \; x = \letexists{a}\congen{M : a} \; \In \;\congen{N : A}
   &\qquad \text{if $M \not\in \dec{GVal}$}
   & \parlab{C-Let} \\

\congen{\Let \; (x : \forall \many{a}. H) = U\; \In \; N : A} &=&
 (\forall \many{a} . \congen{U : H}) \;\wedge\; \Def\; (x: \forall \many{a}. H) \;\In\; \congen{N : A}
 && \parlab{C-LetValAscribe} \\

\congen{\Let \; (x : B) = M\; \In \; N : A} &=&
  \congen{M : B} \;\wedge\; \Def\; (x: B) \;\In\; \congen{N : A}
 & \qquad\text{if $M \not\in \dec{GVal}$}
 & \parlab{C-LetAscribe} \\

\ea
\]

\caption{Constraint generation.}
\label{fig:congen}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/constraint-semantics.tex <==
Use the version in the paper!
\iffalse
\begin{figure}[htbp!]
\raggedright
$\boxed{\Delta; \kenv; \Gamma; \subst \vdash C}$

\begin{mathpar}
\bl
\meta{mostgen}(\Delta, \kenv, \Gamma, \subst, C, \Delta', A', a) = \\
\hspace{0.75cm}%\Delta' = \ftv(A') - \Delta \;\text{ and }\;
(\Delta, \Delta'); (\kenv, a); \Gamma; \subst[a \mapsto A'] \vdash C \;\text{ and }\;\\
\hspace{0.75cm}\bl
(\text{for all }\Delta'', A'' \mid
       \bl
       \text{if }
%       \Delta'' = \ftv(A'') - \Delta \text{ and } \\
       (\Delta, \Delta''); (\kenv, a); \Gamma; \subst[a \mapsto A''] \vdash C \\
       \text{then there exists }
       \rsubst
       \text{ such that } \\
       \;\Delta  \vdash \rsubst : \Delta' \Rightarrow_\poly \Delta''
       \text{ and }
       \rsubst(A') = A'' )\\
       \el \\
\el
\el
\end{mathpar} \\

\begin{mathpar}

\inferrule[\lab{Sem-True}]
  {}
  {\Delta; \kenv; \Gamma; \subst \vdash \dec{true}}

\inferrule[\lab{Sem-And}]
  {
    \Delta; \kenv; \Gamma; \subst \vdash C_1 \\
    \Delta; \kenv; \Gamma; \subst \vdash C_2 \\
  }
  {\Delta; \kenv; \Gamma; \subst \vdash C_1 \wedge C_2}

\inferrule[\lab{Sem-Equiv}]
  {
    \subst(A) = \subst(B)
  }
  {\Delta; \kenv; \Gamma; \subst \vdash A \ceq B}

\inferrule[\lab{Sem-Exists}]
  {
    \Delta \vdash A \\
    \Delta; (\kenv, a : \poly); \Gamma; \subst[a \mapsto A] \vdash C
  }
  {\Delta; \kenv; \Gamma; \subst \vdash \exists a.C}

\inferrule[\lab{Sem-Forall}]
  {
    (\Delta, a); \kenv; \Gamma; \subst \vdash C
  }
  {\Delta; \kenv; \Gamma; \subst \vdash \forall a.C}

\inferrule[\lab{Sem-Instance}]
  {
    \Delta \vdash \many{B} \\
    \Gamma(x) = \forall \many{b}.H \\
    [\many{b} \mapsto \many{B} ](H) = \subst(A)
  }
  {\Delta; \kenv; \Gamma; \subst \vdash x \preceq A}

\inferrule[\lab{Sem-Freeze}]
  {
    \Gamma(x) = \subst(A)
  }
  {\Delta; \kenv; \Gamma; \subst \vdash \freeze{x : A}}

\inferrule[\lab{Sem-Def}]
  {
    \text{for all } a \in \ftv(A) - \Delta: \Delta \vdash \theta(a) : \mono \\
    \Delta; \kenv; (\Gamma,x :  \theta A); \subst \vdash C
  }
  {\Delta; \kenv; \Gamma; \subst \vdash \Def\; (x : A) \;\In\; C}

\inferrule[\lab{Sem-Let}]
  {
    \omany{a} = \ftv(H) - \Delta \\
    A = \forall \omany{a}. H \\\\
    \meta{mostgen}(\Delta, \kenv, \Gamma, \subst, C_1, \many{a}, H, a) \\\\
    a \disjoint \Delta,\many{a} \\
    (\Delta, \many{a}); (\kenv, a : \poly); \Gamma; \subst[a \mapsto H] \vdash C_1 \\
    \Delta; \kenv; (\Gamma,x : A); \subst \vdash C_2
  }
  {\Delta; \kenv; \Gamma; \subst \vdash \Let_\poly\; x = \letexists{a} C_1 \;\In\; C_2}

\inferrule[\lab{Sem-LetMono}]
  {
    \many{a} = \ftv(B) - \Delta \\
%    A = \forall \many{a}. B \\
    \delta = [\many{a} \mapsto \many{S}] \\
    \Delta \vdash \many{S} \\\\
    \meta{mostgen}(\Delta, \kenv, \Gamma, \subst, C_1, \many{a}, B, a)\\\\
    a \disjoint \Delta,\many{a} \\
    (\Delta, \many{a}); (\kenv, a : \poly); \Gamma; \subst[a \mapsto B] \vdash C_1 \\
    \Delta; \kenv; (\Gamma, x : \delta(B)); \subst \vdash C_2
  }
  {\Delta; \kenv; \Gamma; \subst \vdash \Let_\mono\; x = \letexists{a} C_1 \;\In\; C_2}

%% \inferrule[\lab{Sem-LetAsc}]
%%   {
%%     %\Delta \vdash A \\
%%     A = \forall \many{a}. H \\
%%     a \disjoint \Delta, \many{a} \\
%%     (\Delta, \many{a}); (\kenv, a); \Gamma; \subst[a \mapsto H] \vdash C_1 \\
%%     \Delta; \kenv; (\Gamma,x : A); \subst \vdash C_2
%%   }
%%   {\Delta; \kenv; \Gamma; \subst \vdash \Let\; (x : A) = \letexists{a} C_1 \;\In\; C_2}

%% \inferrule[\lab{Sem-LetMonoAsc}]
%%   {
%%     %\Delta \vdash A \\
%%     a \disjoint \Delta \\
%%     \Delta; (\kenv, a); \Gamma; \subst[a \mapsto A] \vdash C_1 \\
%%     \Delta; \kenv; (\Gamma,x : A); \subst \vdash C_2
%%   }
%%   {\Delta; \kenv; \Gamma; \subst \vdash \Let_\mono\; (x : A) = \letexists{a} C_1 \;\In\; C_2}

\end{mathpar}

\caption{Semantics of constraints.}
\label{fig:contraints-semantics}
\end{figure}
\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/constraint-syntax.tex <==
\begin{figure}[ht]

\[
\bl
\ba[t]{@{}l@{\quad}r@{~}c@{~}l@{}}
\slab{Constraints}            &\dec{Constr} \ni C &::= &
                                        \dec{true}
                                   \mid C \wedge C
                                   \mid A \ceq B
                                   \mid \exists a.C
                                   \mid x \preceq A
                                   \mid \freeze{x : A}
                                   \mid \forall a. C
                                   \mid \Def\; (x : A) \;\In\; C\\
                           &&\mid& \Let_\poly\; x = \letexists{a} C \;\In\; C
%                                   \mid \Let\phantom{_\mono}\; (x : A) = \letexists{a} C \;\In\; C \\
                            \mid \Let_\mono\; x = \letexists{a} C \;\In\; C\\
%                                   \mid \Let_\mono\; (x : A) = \letexists{a} C \;\In\; C \\

\slab{Restriction}            &\dec{Restr} \ni R &::= & \mono \mid \poly
\ea \\
\el
\]

\caption{Constraints Syntax.}
\label{fig:constraints-syntax}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/constraint-wellformedness.tex <==
\begin{figure}[h]
\raggedright
$\boxed{\Delta;\Xi;\Gamma \vdash \wf{C}}$

\begin{mathpar}

\inferrule[\lab{WF-Constr-True}]
  { }
  {\Delta; \Xi; \Gamma \vdash \wf{\dec{true}}}

\inferrule[\lab{WF-Constr-Mono}]
  { }
  {\Delta; (\Xi, a); \Gamma \vdash \wf{\monoc(a)}}

\inferrule[\lab{WF-Constr-And}]
  {\Delta; \Xi; \Gamma \vdash \wf{C_1}\\
   \Delta; \Xi; \Gamma \vdash \wf{C_2}}
  {\Delta; \Xi; \Gamma \vdash \wf{C_1 \wedge C_2}}

\inferrule[\lab{WF-Constr-Exist}]
  {\Delta; (\Xi, a); \Gamma \vdash \wf{C}}
  {\Delta; \Xi; \Gamma \vdash \wf{\exists a. C}}

\inferrule[\lab{WF-Constr-Forall}]
  {(\Delta, \many{a}); \Xi; \Gamma \vdash \wf{C}}
  {\Delta; \Xi; \Gamma \vdash \wf{\forall \many{a}. C}}

\inferrule[\lab{WF-Constr-Equiv}]
  {(\Delta, \Xi) \vdash \wf{A}\\
   \Delta, \Xi \vdash B}
  {\Delta; \Xi; \Gamma \vdash \wf{A \ceq B}}

\inferrule[\lab{WF-Constr-Instance}]
  {x \in \Gamma\\
   (\Delta, \Xi) \vdash \wf{A}}
  {\Delta; \Xi; \Gamma \vdash \wf{x \preceq A}}

\inferrule[\lab{WF-Constr-Freeze}]
  {x \in \Gamma\\
   (\Delta, \Xi) \vdash \wf{A}}
  {\Delta; \Xi; \Gamma \vdash \wf{\freeze{x : A}}}

\inferrule[\lab{WF-Constr-Def}]
  {(\Delta, \Xi) \vdash \wf{A} \\
   \Delta; \Xi; (\Gamma, x : A) \vdash \wf{C}}
  {\Delta; \Xi; \Gamma \vdash \wf{\Def\; (x : A) \;\In\; C}}

\inferrule[\lab{WF-Constr-Let}]
  {\Delta;  (\Xi, a); \Gamma \vdash \wf{C_1}\\\\
   \Delta; \Xi; (\Gamma, x : A) \vdash \wf{C_2}}
  {\Delta; \Xi; \Gamma \vdash \wf{\Let_R \; x = \letexists{a} C_1 \;\In\; C_2}}

\end{mathpar}

\caption{Constraint Well-formedness.}
\label{fig:contraints-wellformedness}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/freezeml-aux.tex <==
\begin{figure}[tb]
\raggedright
$\boxed{\Delta \vdash \rsubst : \Delta' \Rightarrow_R \Delta''}$
\begin{mathpar}
\inferrule
  { }
  {\Delta \vdash \emptyset : \cdot \Rightarrow_R \Delta'}

\inferrule
  {\Delta \vdash \rsubst : \Delta' \Rightarrow_R \Delta'' \\
   \Delta, \Delta'' \vdash_R \wf{A}}
  {\Delta \vdash \rsubst[a \mapsto A] : (\Delta', a) \Rightarrow_R \Delta''}
\end{mathpar}

$\boxed{(\Delta, \omany{a}, M, A') \Updownarrow A}$
\begin{mathpar}
\inferrule
  {M \in \dec{GVal}}
  {(\Delta, \omany{a}, M, A') \Updownarrow \forall \omany{a}. A'}

\inferrule
  {\Delta' = \many{a} \\
   \Delta \vdash \rsubst : \Delta' \Rightarrow_\mono \cdot \\ M \not\in \dec{GVal}}
  {(\Delta, \omany{a}, M, A') \Updownarrow \rsubst(A')}
\end{mathpar}


\begin{mathpar}
\bl
\meta{split}(\forall \omany{a}.H, M) =
\left\{
\ba{@{~}l@{}@{\quad}l}
  (\many{a}, H)              & \text{if $M \in \dec{GVal}$} \\
  (\cdot,\forall \omany{a}.H) & \text{otherwise}
\ea
\right.
\el

\end{mathpar}
\begin{mathpar}
\bl
\meta{principal}(\Delta, \Gamma, M, \Delta', A') = \\
\qquad
\Delta, \Delta'; \Gamma \vdash M : A' \;\text{ and } \\
\qquad\bl
(\text{for all }\Delta'', A'' \mid
       \bl
       \text{if }
%       \Delta'' = \ftv(A'') - \Delta \text{ and } \\
       \Delta, \Delta''; \Gamma \vdash M : A'' \\
       \text{then there exists }
       \rsubst
       \text{ such that } \\
       \;\Delta  \vdash \rsubst : \Delta' \Rightarrow_\poly \Delta''
       \text{ and }
       \rsubst(A') = A'' )\\
       \el \\
\el
\el
\end{mathpar}
\caption{\freezeml Auxiliary Definitions.}
\label{fig:freezeml-aux-judgments}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/freezeml-syntax.tex <==
\begin{figure}[ht]

\[
\bl
\ba[t]{@{}l@{}r@{~}c@{~}l@{}}
\slab{Type Variables}         &\dec{TVar} \ni a, b, c \\
%% \slab{Skolem Variables}       &\dec{SVar} \ni \skolem{a}, \skolem{b}, \skolem{c}&\\
\slab{Type Constructors}      &\dec{Con}  \ni D &::= &
                                        \mathord{\to}
                                   \mid \times
                                   \mid \Int
                                   \mid \dots \\
\slab{Types}                  &\dec{Type} \ni A, B      &::= &
                                         a
                                    \mid D\,\many{A}
                                    \mid \forall a.A \\
\slab{Monotypes}              &\dec{MType} \ni S, T      &::= &
                                         a
                                    \mid D\,\many{S} \\
\slab{Guarded Types}          &\dec{GType} \ni H &::= &
                                         a
                                    \mid D\,\many{A} \\
\slab{Type Instantiation}     &\dec{Subst} \ni \rsubst  &::= &
                                          \emptyset \mid \rsubst[a \mapsto A] \\
\slab{Type Substitutions}     &\dec{Subst} \ni \subst  &::= &
                                          \emptysubst \mid \subst[a \mapsto A] \\
\slab{Kinds}                  &\dec{Kind} \ni \kappa&::= & \mono \mid \poly \\
\slab{Kind Environments}      &\dec{KEnv} \ni \Delta    &::= &
                                        \cdot \mid \Delta, a\\
\slab{Type Environments}      &\dec{TEnv} \ni \Gamma    &::= &
                                          \cdot \mid \Gamma, x : A \\
\slab{Term Variables}         &\dec{Var} \ni x, y, z \\
\slab{Terms}                  &\dec{Term} \ni M, N      &::= &
                                        x
                                   \mid \freeze{x}
                                   \mid \lambda x. M
                                   \mid \lambda (x : A). M
                                   \mid M\,N \\
                           &&\mid& \Let\; x = M \;\In\; N
                                   \mid \Let\; (x : A) = M \;\In\; N
                                   \mid \dots
                                   \\
\slab{Values}                 &\dec{Val} \ni V, W       &::= &
                                        x
                                   \mid \freeze{x}
                                   \mid \lambda x.M
                                   \mid \lambda (x : A). M\\
                           &&\mid& \Let\; x = V \;\In\; W
                                   \mid  \Let\; (x : A) = V \;\In\; W \\
\slab{Guarded Values}         &\dec{GVal} \ni U       &::= &
                                        x
                                   \mid \lambda x.M
                                   \mid \lambda (x : A). M\\
                           &&\mid& \Let\; x = V \;\In\; U
                                   \mid  \Let\; (x : A) = V \;\In\; U \\
\ea \\
\el
\]

\caption{FreezeML Syntax.}
\label{fig:syntax}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/gamma-wellformedness.tex <==
% \begin{figure}[htb]
% \raggedright
% $\boxed{\Delta;\kenv \vdash \wf{\Gamma}}$

\begin{mathpar}

\inferrule%[\lab{WF-Gamma-Empty}]
  { }
  {\Delta \vdash \wf{\emptygamma}}

\inferrule%[\lab{WF-Gamma-Cons}]
  {\Delta \vdash \wf{A}\\
   \Delta \vdash \wf{\Gamma}}
  {\Delta \vdash \wf{\Gamma, x : A}}


\end{mathpar}

% \caption{Term context well-formedness.}
% \label{fig:gamma-wellformedness}
% \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/preservation-aux.tex <==
\begin{figure}[htb]

\[
\bl
\ba[t]{@{}r@{~}c@{~}l}
F_\emptygamma &=& \emptystack\\

F_{\Gamma, x : A} &=& \Def\;x : A :: F_\Gamma\\


\ea \\
\el
\]
\fe{The definition of $F_\Gamma$ above doesn't seem to be used anywhere.  }


\caption{Auxiliary Definitions.}
\label{fig:preservation-aux}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/stack-context-plugging.tex <==
\begin{figure}[h]

\[
\bl
\ba[t]{@{}r@{\quad}c@{\quad}l@{\quad}r@{}}

\emptystack[C] &=& C & (\lab{SC-Empty})\\[2pt]

(F :: \Box \wedge C_2)[C_1] &=& F[C_1 \wedge C_2] & (\lab{SC-Conj})\\[2pt]

(F :: \forall\; a)[C] &=& F[\forall a. C] & (\lab{SC-Forall})\\[2pt]

(F :: \exists\; a)[C] &=& F[\exists a. C] & (\lab{SC-Exists})\\[2pt]

(F :: \Let_R\, x = \letexists{a} \Box \;\dec{in}\; C_2 )[C_1] &=&
F[\Let_R\, x = \letexists{a} C_1 \;\In\; C_2] &
(\lab{SC-Let})\\[2pt]

(F :: \Def\; (x : A) )[C] &=& F[\Def\; (x : A) \;\In\; C] & (\lab{SC-Def})\\[2pt]

\ea
\el
\]

\caption{Stack Context Plugging.}
\label{fig:stack-context-plugging}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/stack-machine-aux.tex <==
\begin{figure}[htb]
\fe{Note that in the following, we must apply the fist equation that matches.}

\[
\bl
\ba[t]{@{}r@{~}c@{~}l}

\fv(\emptystack) &=& \emptyset\\

\fv(F :: \Box \wedge C) &=& \fv(C) \cup \fv(F)\\

\fv(F :: \Let_R\, x = \letexists{a}\Box \;\dec{in}\; C ) &=& \fv(C) \setminus \lbrace x \rbrace \cup \fv(F)\\

\fv(F :: \_ ) &=& \fv(F)\\\\

\btv(\emptystack) &=& \emptyset\\

\btv(F :: \Box \wedge C ) &=& \btv(C) \cup \btv(F)\\

\btv(F :: \Let_R\, x = \letexists{a}\Box \;\dec{in}\; C ) &=& \lbrace a \rbrace \cup \btv(C) \cup \btv(F)\\

\btv(F :: \exists a) &=& \lbrace a \rbrace \cup \btv(F)\\

\btv(F :: \forall a) &=& \lbrace a \rbrace \cup \btv(F)\\

\btv(F :: \_ ) &=& \btv(F) \\\\


\dec{split}(\many{a}, \theta, \Theta) &=& \many{b} ; \many{c} \\
&&\text{where }
\bl
\ba[t]{@{}l}
\many{b}, \many{c} = \many{a} \\
\text{for all } c \in \many{a}: c \in \many{c} \text{ iff } c \in \ftv(\theta(\Theta - \many{a}))
\ea
\el
\\

\ea \\
\el
\]

\caption{Constraint Solving Using Stack Machines: Auxiliary Definitions.}
\label{fig:contraints-stack-machine-aux}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> figures/stack-machine-syntax.tex <==
\begin{figure}[ht]

\[
\bl
\ba[t]{@{}l@{\quad}r@{~}c@{~}l@{}}
%% \slab{Restrictions}           &\dec{Restr} \ni R&::=&
%%                                         \cdot
%%                                    \mid \mono\\
\slab{Frames}                 &\dec{Frm} \ni f         &::= &
                                        \Box \wedge C
                                   \mid \forall\; a
                                   \mid \exists\; a
                                   \mid \Let_R \; x = \letexists{a} \Box \;\dec{in}\; C
                                   \mid \Def\; (x : A) \\
\slab{Stack}                  &\dec{Stk} \ni f         &::= &
                                        \emptystack
                                   \mid F :: f\\
\slab{Flexible Environments}  &\dec{FEnv} \ni \kenv &::=&
                                        \emptykenv
                                   \mid \kenv, a : \kappa\\
\slab{States}                 &\dec{St} \ni s          &::= &
                                        (F, \kenv, \subst, C)\\
\ea \\
\el
\]

\caption{Constraints Stack Machine Syntax.}
\label{fig:constraint-stack-machine-syntax}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "constraint_freezeml"
%%% End:


==> proofs/aux-proofs.tex <==
\stackcontextwf*
% Proof:
\input{proofs/stack-context-well-formed.tex}

\unificationthetaequiv*

\input{proofs/stack-context-well-formed.tex}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> proofs/semantics-equiv-stack-machine.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% PROOF OF THEOREM 5:  ∆;Γ;φ |- C  <=> (φ,Γ,F,C)  →∗ (φ',Γ,F,true)           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\todo{Remove generating fresh variables from S1 exists and let rules?  Make a
  todo note for the two remaining stack machines.}

\todo{Figure out the exact placement of quantifiers in proof statement.}

\todo{Let cases are completely broken at the moment.}

\constraintssolvableunifybysubstnorank*

\begin{proof}
We prove $\Rightarrow$ direction by induction on the derivation of
$\Delta;\Gamma;\subst\vdash C$ defined in Figure~\ref{fig:contraints-semantics}.

\begin{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash \true$

\proofContext{sem-stack-equiv-true-case}

Immediate.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash C_1 \wedge C_2$

\proofContext{sem-stack-equiv-conj-case}

Premisses and inductive hypotheses:

\begin{premisses}
 \item $\forall K. (\subst,\Gamma,F,C_1) \to^{*} (\subst,\Gamma,F,\true)$
   \premissLabel{ih1}
 \item $\forall K. (\subst,\Gamma,F,C_2) \to^{*} (\subst,\Gamma,F,\true)$
   \premissLabel{ih2}
\end{premisses}

\[
\ba[t]{r@{\quad}c@{\quad}l}
(\subst,\Gamma,F,C_1 \wedge C_2)

 &\from{\lab{S-ConjIn}} &
     (\subst,\Gamma,\Box \wedge C_2 :: F,C_1)\\

 &\from{\premissRef{ih1}} &
     (\subst,\Gamma,\Box \wedge C_2 :: F, \true)\\

 &\from{\lab{S-ConjOut}} &
     (\subst,\Gamma, F, C_2)\\

 &\from{\premissRef{ih2}} &
     (\subst,\Gamma, F, \true)\\
\ea
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash A \ceq B$

\proofContext{sem-stack-equiv-eq-case}

Premisses and inductive hypotheses:

\begin{premisses}
 \item $\subst(A) = \subst(B)$ \premissLabel{type-eq}
\end{premisses}

\[
\ba[t]{r@{\quad}c@{\quad}l}
(\subst,\Gamma,F, A \ceq B)

 &\from{\lab{S-Eq}} &
     (\substunifier(\subst A, \subst B) \comp \subst, \Gamma, F, \true)\\

 &\from{\text{rewrite }\premissRef{type-eq}} &
     (\substunifier(\subst B, \subst B) \comp \subst, \Gamma, F, \true)\\

 &\from{\lab{US-Refl}} &
     (\subst,\Gamma, F, \true)\\
\ea
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash \exists a. C$

\proofContext{sem-stack-equiv-exists-case}

Premisses and inductive hypotheses:

\begin{premisses}
 \item $\forall K. (\subst[a \mapsto A], \Gamma, F, C) \to^{*} (\subst[a
   \mapsto A], \Gamma, F, \true)$ \premissLabel{ih}
\end{premisses}

\[
\ba[t]{r@{\quad}c@{\quad}l}
(\subst, \Gamma, F, \exists a. C)

 &\from{\lab{S-Exists}} &
     (\subst, \Gamma, F, C)\\

 &\from{\phantom{Ly}} & \js{\text{What now?}}\\
\ea
\]

\js{Inductive hypothesis does not apply here.  Ideas?  Can $A$ in IH be
  considered universally quantified?  If so we can do this:}

\[
\ba[t]{r@{\quad}c@{\quad}l}
(\subst, \Gamma, F, \exists a. C)

 &\from{\lab{S-Exists}} &
     (\subst, \Gamma, F, C)\\

 &\from{\phantom{Ly}} &
     (\subst[a \mapsto a], \Gamma, F, C)\\

 &\from{\premissRef{ih}} &
     (\subst[a \mapsto a], \Gamma, F, \true)\\
\ea
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash x \preceq A$

\proofContext{sem-stack-equiv-inst-case}

Premisses and inductive hypotheses:

\begin{premisses}
 \item $\Gamma(x) = \forall\many{b}.B$ \premissLabel{in-gamma}
 \item $\subst[\many{b} \mapsto \many{B}](B) = \subst(A)$ \premissLabel{subst}
\end{premisses}

\[
\ba[t]{r@{\quad}c@{\quad}l}
(\subst, \Gamma, F, A \preceq B)

 &\from{\lab{S-Inst}} &
     (\subst, \Gamma, F, [\many{a}/\many{b}]B \ceq A)\\

 &\from{\phantom{Ly}} &
     (\subst[\many{b}\mapsto\many{a}], \Gamma, F, B \ceq A)\\

 &\from{\lab{S-Eq}} &
     (\substunifier(\subst[ \many{b} \mapsto \many{a}] B,
                    \subst[ \many{b} \mapsto \many{a}] A) \comp
                    \subst[ \many{b} \mapsto \many{a}],
                  \Gamma, F, \true)\\
\ea
\]

We now need to prove that unification
$\substunifier(\subst[\many{b}\mapsto\many{a}]B,
\subst[\many{b}\mapsto\many{a}]A)$ does not fail.  Since $\many{b}$ are
quantifiers of $B$ they are absent from $A$, which allows to simplify to
$\substunifier(\subst[\many{b}\mapsto\many{a}]B, \subst A)$.  We now rewrite
$\subst A$ using premiss \premissRef{subst} to obtain
$\substunifier(\subst[\many{b}\mapsto\many{a}]B,
\subst[\many{b}\mapsto\many{B}](B))$.  From $\lab{US-Type}$ unification rule we
know all $\many{a}$ will unify with corresponding $\many{B}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash \freeze{x : A}$

\proofContext{sem-stack-equiv-freeze-case}

Premisses and inductive hypotheses:

\begin{premisses}
 \item $\Gamma(x) = \subst(A)$ \premissLabel{in-gamma} \js{Wrong?}
\end{premisses}

\[
\ba[t]{r@{\quad}c@{\quad}l}
(\subst, \Gamma, F, \freeze{x : A})

 &\from{\lab{S-Freeze}} & (\subst'', \Gamma, F, \true)\\

\ea
\]

where $\subst'' = \lbrack \many{\skolem{b}} \mapsto \many{b} \rbrack \comp
\substunifier(\subst' A,\subst'(\forall\many{b}.B)) \comp \subst'$ and $\lbrack
\many{b} \mapsto \many{\skolem{b}} \rbrack \comp \subst$.  We now need to prove
that $\substunifier(\subst' A,\subst'(\forall\many{b}.B))$ does not fail.  Since
quantifiers $\many{b}$ don't appear in $A$ we can rewrite $\subst' A$ to $\subst
A$ and then rewrite using premiss \premissRef{in-gamma} to obtain
$\substunifier(\Gamma(x),\subst'(\forall\many{b}.B))$, which further rewrites to
$\substunifier(\forall\many{b}.B,\subst'(\forall\many{b}.B))$

\js{This proof can only be finished if \premissRef{in-gamma} says
  $\subst(\Gamma(x)) = \subst(A)$ \label{temp:freeze-rule-needs-fix}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash \Let_\mono \; x = \letexists{a}C_1 \; \In
  \;C_2$

\proofContext{sem-stack-equiv-let-mono-case}

Premisses and inductive hypotheses:

\begin{premisses}
 \item $(\Delta, \many{a}); \Gamma; \subst[ a \mapsto B ] \vdash C_1$
   \premissLabel{c1-wellformed}
 \item %$(\Delta, \many{a}); \Gamma; \subst[ a \mapsto B ] \vdash C_1 \Rightarrow
   $\forall K. (\subst[a \mapsto B], \Gamma, F, C_1) \to^{*} (\subst'[a \mapsto
   \js{?}], \Gamma, F, \true)$ \premissLabel{ih-c1}
 \item $\Delta; (\Gamma, x : \delta(B)); \subst \vdash C_2$
   \premissLabel{c2-wellformed}
 \item %$\Delta; (\Gamma, x : \delta(B)); \subst \vdash C_2 \Rightarrow$
   $\forall K. (\subst, (\Gamma, x : \delta(B)), F, C_2) \to^{*} (\subst',
   (\Gamma, x : \delta(B)), F, \true)$ \premissLabel{ih-c2}
\end{premisses}

\js{In the above premisses $B$ is a type that semantic rule $\lab{Sem-LetMono}$
  pulls out of thin air.  This is problematic if we want to use
  \premissRef{ih-c1} as premiss to
  Lemma~\ref{lemma:aux:solver-finds-principal-type} since it requires $[a
    \mapsto a]$, not $[a \mapsto B]$.  I believe we can validly argue that if
  $B$ is pulled out of thin air by the rule then it should really be a fresh
  unification variable that the solver makes precise.  How do we make this
  reasoning precise?}

\js{Below I assume that $\lab{S-LetInMono}$ does not generate a fresh variable
  $b$ to substitute in $C_1$.  This allows to apply
  Lemma~\ref{lemma:aux:solver-finds-principal-type}, which demands $\subst[a
    \mapsto a]$, not $\subst[a \mapsto b]$.  Alternatively we can keep the
  freshness requirement and then rewrite $\subst[a \mapsto b]$ to $\subst[a
    \mapsto b][b \mapsto b]$.  It is also worth having a substitution
  transitivity law that would allow us to then shorten the result from $\subst[a
    \mapsto b][b \mapsto B]$ to $\subst[a \mapsto B]$.}

\js{Following reasoning is wrong and was based on my mistake in writing down
  Lemma~\ref{lemma:aux:solver-finds-principal-type}.}

\[
\ba[t]{r@{\quad}c@{\quad}l}
(\subst, \Gamma, F, \Let_\mono \; x = \letexists{a}C_1 \; \In \;C_2)

 &\from{\lab{S-Let}} &
     ([a \mapsto a] \comp \subst, \Gamma, \dec{let}_\mono \; x = a  \,\dec{in}\, C_2 :: F, C_1)\\

 &\from{\premissRef{c1-wellformed}, \text{ Lemma }\ref{lemma:aux:solver-finds-principal-type}} &
     ([a \mapsto A] \comp \subst,
      \Gamma, \dec{let}_\mono \; x = a  \,\dec{in}\, C_2 :: F, \true)\\

 &\from{\lab{S-LetInMono}} &
     ([\many{a'} \mapsto \many{a'_\mono}] \comp [a \mapsto A] \comp \subst,
      (\Gamma, x : A), \dec{let} :: F, C_2)\\
 &&\small{\text{where $\many{a'} \leftarrow \mgen_\Gamma(B) $}} \\

 &\from{\premissRef{ih-c2}} &
     ([\many{a'} \mapsto \many{a'_\mono}] \comp [a \mapsto A] \comp \subst,
      (\Gamma, x : A), \dec{let} :: F, \true)\\

 &\from{\lab{S-DefOut}} &
     ([\many{a'} \mapsto \many{a'_\mono}] \comp [a \mapsto A] \comp \subst, \Gamma, F, \true)\\
\ea
\]

\todo{When we use premiss \premissRef{ih-c2} we have to prove equivalence
  between $\delta(B)$ in \premissRef{ih-c2} and $A$ in current proof state.
  From conclusion of Lemma~\ref{lemma:aux:solver-finds-principal-type} we know
  $\delta(B)$ is an instance of $A$.  Does that suffice?  Moreover, $\subst$ is
  fixed in \premissRef{ih-c2} and does not match $[\many{a'} \mapsto
    \many{a'_\mono}] \comp [a \mapsto A] \comp \subst$ in the actual proof
  state.  Here's a reasoning that might fix this.  $a$ was only bound in $C_1$.
  Since $C_1$ was solved we should be able to throw away $[a \mapsto A]$
  substitution since $a$ does not appear anywhere else.  That however is a
  non-trivial lemma since it's not immediately obvious that solving $C_1$ did
  not made copies of $a$ inside $\subst'$.  The $[\many{a'} \mapsto
    \many{a'_\mono}]$ part ensures that free variables in $A$ are only
  substituted in a monomorphic way, which is what $\delta(B)$ does.  The
  important difference is that $\delta$ pulls types out of thin air whereas the
  stack machine leaves these types to be discovered later.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash \Let_\poly \; x = \letexists{a}C_1 \; \In
  \;C_2$

\proofContext{sem-stack-equiv-let-case}

Premisses and inductive hypotheses:

\begin{premisses}
 \item $(\Delta, \many{a}); \Gamma; \subst[ a \mapsto H ] \vdash C_1$
   \premissLabel{c1-wellformed}
 %% \item $\Delta; (\Gamma, x : \forall \many{a}. H); \subst \vdash C_2$
 %%   \premissLabel{c2-wellformed}
 \item %$\Delta; (\Gamma, x : \forall \many{a}. H); \subst \vdash C_2 \Rightarrow$
  $\forall K. (\subst, (\Gamma, x : \forall \many{a}. H), F, C_2) \to^{*}
   (\subst', (\Gamma, x : \forall \many{a}. H), F, \true)$ \premissLabel{ih}
\end{premisses}

\js{Below I assume that $\lab{S-LetIn}$ does not generate a fresh variable $b$ to
  substitute in $C_1$.  This allows to apply
  Lemma~\ref{lemma:aux:solver-finds-principal-type}, which demands $\subst[a
    \mapsto a]$, not $\subst[a \mapsto b]$.}

\[
\ba[t]{r@{\quad}c@{\quad}l}
(\subst, \Gamma, F, \Let_\poly \; x = \letexists{a}C_1 \; \In \;C_2)

 &\from{\lab{S-Let}} &
     (\subst, \Gamma, \dec{let} \; x = a  \,\dec{in}\, C_2 :: F, C_1)\\

 &\from{\phantom{Ly}} &
     ([a \mapsto a] \comp \subst,
      \Gamma, \dec{let} \; x = a  \,\dec{in}\, C_2 :: F, C_1)\\

 &\from{\premissRef{c1-wellformed}, \text{ Lemma }\ref{lemma:aux:solver-finds-principal-type}} &
     ([a \mapsto B] \comp \subst ,
      \Gamma, \dec{let} \; x = a  \,\dec{in}\, C_2 :: F, \true)\\

 &\from{\lab{S-LetIn}} &
     ([a \mapsto B] \comp \subst,
      (\Gamma, x : \forall \many{a}.[\many{a} / \mgen_\Gamma(B)] B), \dec{let} :: F, C_2)\\

 &\from{\premissRef{ih}} &
     ([a \mapsto B] \comp \subst,
      (\Gamma, x : \forall \many{a}.[\many{a} / \mgen_\Gamma(B)] B),
      \dec{let} :: F, \true)\\

 &\from{\lab{S-DefOut}} &
     ([a \mapsto B] \comp \subst, \Gamma, F, \true)\\
\ea
\]

\todo{When we use premiss \premissRef{ih} we have to prove equivalence between
  $\forall \many{a}. H$ in \premissRef{ih} and $\forall \many{a}.[\many{a} /
    \mgen_\Gamma(B)] B$ in current proof state.  From conclusion of
  Lemma~\ref{lemma:aux:solver-finds-principal-type} we know $H$ is an instance of $B$.
  Does that suffice?}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash \Let_\mono \; (x : A) = \letexists{a}C_1
  \; \In \;C_2$

\proofContext{sem-stack-equiv-let-mono-asc-case}

Premisses and inductive hypotheses:

\begin{premisses}
 \item $\Delta; \Gamma; \subst[a \mapsto A] \vdash C_1$
   \premissLabel{c1-wellformed}
 \item %$\Delta; (\Gamma, x : \forall \many{a}. H); \subst \vdash C_2 \Rightarrow$
  $\forall K. (\subst, (\Gamma, x : A), F, C_2) \to^{*} (\subst', (\Gamma, x :
   A), F, \true)$ \premissLabel{ih}
\end{premisses}

\[
\ba[t]{r@{\quad}c@{\quad}l}
(\subst, \Gamma, F, \Let_\mono \; (x : A) = \letexists{a}C_1 \; \In \;C_2)

 &\from{\lab{S-LetAsc}} &
     ([a \mapsto a] \comp \subst,
      \Gamma, \dec{let}_\mono \; x : A = a  \,\dec{in}\, C_2 :: F, C_1)\\

 &\from{\premissRef{c1-wellformed}, \text{ Lemma }\ref{lemma:aux:solver-finds-principal-type}} &
     ([a \mapsto A'] \comp \subst,
      \Gamma, \dec{let}_\mono \; x : A = a  \,\dec{in}\, C_2 :: F, \true)\\

 &\from{\lab{S-LetInMonoAsc}} &
     (\subst'' \comp [a \mapsto A'] \comp \subst,
      (\Gamma, x : A), \dec{let} :: F, C_2)\\

 &\from{\phantom{Ly}} &
     \todo{\text{define $\subst''$, prove unification does not fail}}\\

 &\from{\premissRef{ih}} &
     (\subst'' \comp [a \mapsto A'] \comp \subst,
      (\Gamma, x : A), \dec{let} :: F, \true)\\

 &\from{\lab{S-DefOut}} &
     (\subst'' \comp [a \mapsto A'] \comp \subst, \Gamma, F, \true)\\

\ea
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Case $\Delta; \Gamma; \subst \vdash \Let_\poly \; (x : A) = \letexists{a}C_1 \; \In
  \;C_2$

\proofContext{sem-stack-equiv-let-asc-case}

\todo{Same as above three cases.  Once we figure out all the details this case
  will be analogous.}

\end{itemize}

\end{proof}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:


==> proofs/stack-context-well-formed.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PROOF OF WELL-FORMEDNESS OF STACK CONTEXT PLUGGING:                          %
%                                                                              %
%        Δ;Θ;Γ ⊢ C ok ∧ Δ;Θ;Γ ⊢ F ok ⇔ Δ_F;Θ_F;Γ ⊢ F[C] ok                     %
%                                                                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}
\proofContext{stack-context-well-formed}

%
By induction on the derivation of
$\Delta; \kenv; \Gamma \vdash \wf{F}$, as defined in
Figure~\ref{fig:stack-wellformedness}.
%
Theorem premisses:

\begin{premisses}
  \item $\btv(F) \disjoint \btv(C)$ \premissLabel{premiss:btv-c-f-disjoint}
  \item $\Delta; \kenv; \Gamma \vdash \wf{C}$ \premissLabel{premiss:c-wf}
\end{premisses}

For an empty stack (case $\lab{WF-Stack-Empty}$), the desired property follows
immediately.
Otherwise, the stack of $F$ is of the form $f :: F'$.
We observe that $(f :: F')[C] = F'[ (f::\cdot)[C] ]\: \premissNum{premiss:wf-c}$
holds, and abbreviate $(f::\cdot)[C]$ as $f[C]$.
\begin{itemize}
\item Case $\lab{WF-Stack-Conj}$:
We have a derivation of the form
\[
\inferrule
  {
   \btv(C') \disjoint \btv(F') \\\\
   \Delta; \kenv; \Gamma \vdash \wf{C'} \\
   \Delta; \kenv; \Gamma \vdash \wf{F'}}
  {\Delta; \kenv; \Gamma \vdash \wf{\Box \wedge C' :: F'}}
\]

with $f = \Box \wedge C'$ and $f[C] = C \wedge C'$.

We have $\btv(C') \subseteq \btv(F)$,
which in conjunction with premiss
\premissRef{premiss:btv-c-f-disjoint} implies
$\btv(C) \disjoint \btv(C')$~\premissLabel{btv-C-Cprime-disj}.
We can now derive
\[
\inferrule
  {\btv(C) \disjoint \btv(C')\\\\
   \Delta; \kenv; \Gamma \vdash \wf{C}\\
   \Delta; \kenv; \Gamma \vdash \wf{C'}}
  {\Delta; \kenv; \Gamma \vdash \wf{C \wedge C'}}
\]

By $\btv(C') \disjoint \btv(F')$ we have
as $\btv(F) = \btv(F') \uplus \btv(C')$.
We can therefore re-state
\premissRef{premiss:btv-c-f-disjoint} as $\btv(F') \uplus \btv(C') \disjoint \btv(C)$,
which implies
$\btv(F') \disjoint \btv(C) \cup \btv(C')$.
We have $\btv(f[C]) = \btv(C) \cup \btv(C')$, which gives us
$\btv(F') \disjoint \btv(f[C])$~\premissNum{btv-Fprime-fC-disj}.

Applying the induction hypothesis to
$\Delta; \kenv; \Gamma \vdash \wf{F'}$ and
$\Delta;\Theta;\Gamma \vdash \wf{f[C]}$ and
\premissRef{btv-Fprime-fC-disj}
yields
$\resd{\Delta}{F'},\resk{\kenv}{F'},\resd{\Gamma}{F'} \vdash \wf{F'[f[C]]}$
\premissNum{premiss:f-c-prim-wf}.
%
By definitions in Figure~\ref{fig:preservation-aux} we have
$\resd{\Delta}{F}$ = $\resd{\Delta}{F'}$
$\resk{\kenv}{F}$ = $\resk{\kenv}{F'}$,
$\resd{\Gamma}{F}$ = $\resd{\Gamma}{F'}$.
Rewriting \premissRef{premiss:f-c-prim-wf} by
$\premissRef{premiss:wf-c}$
we obtain the desired property
$\resd{\Delta}{F};\resk{\kenv}{F}; \resg{\Gamma}{F} \vdash \wf{F[C]}$.


\item Case $\lab{WF-Stack-Forall}$:
We have a derivation of the form
\[
\inferrule
  {
   \Delta'; \kenv; \Gamma \vdash \wf{F'}}
  {(\Delta', \many{a}); \kenv; \Gamma \vdash \wf{\forall \; \many{a} :: F'}}
\]
where $\Delta = (\Delta', \many{a})$
and can derive
\[
\inferrule
  {
   (\Delta', \many{a}) ; \kenv; \Gamma \vdash \wf{C}}
  {\Delta' ; \kenv; \Gamma \vdash \wf{\forall \many{a}. C}}
\]

\fe{It seems somewhat weird that the well-formedness rule doesn't impose
  $\ftv(\Gamma) \disjoint \many{a}$. The corresponding rule in the semantics of
  constraints judgement does, though.}
%
\js{Semantic rule imposes this implicitly by asserting that whenever $\Delta;
  \kenv; \Gamma; \subst \vdash C$ holds it is the case that $\ftv(\Gamma)
  \subseteq \Delta$.  Should we add similar implicit assumptions to $\Delta;
  \kenv; \Gamma \vdash \wf{C}$?  I think it doesn't make sense to talk about
  well-formedness of $C$ in the context of $\Gamma$ unless $\Gamma$ itself is
  well-formed.}

We have $\btv(F) = \btv(F')$ and $\btv(C) = \btv(f[C])$.
This means that \premissRef{premiss:btv-c-f-disjoint} implies
$\btv(F') \disjoint \btv(f[C])$~\premissNum{forall:btv-Fprime-vs-fC}.

Applying the induction hypothesis to $\Delta'; \kenv; \Gamma \vdash \wf{F'}$ and
$\Delta';\Theta;\Gamma \vdash \wf{f[C]}$ and \premissRef{forall:btv-Fprime-vs-fC}
 gives us $\resd{\Delta'}{F'};
\resk{\kenv}{F'}; \resg{\Gamma}{F'} \vdash F'[f[C]]$.
We have
$\resd{\Delta}{F}$ = $\resd{\Delta'}{F'}$
$\resk{\kenv}{F}$ = $\resk{\kenv}{F'}$, and
$\resd{\Gamma}{F}$ = $\resd{\Gamma}{F'}$,
which makes this equivalent to the desired property.

\item Case $\lab{WF-Stack-Let}$:
We have a derivation of the form
\[
\inferrule
  {
   \{ a \} \uplus \btv(C') \disjoint \btv(F')\\
   \Delta; (\kenv', a : \poly); (\Gamma, x : \bot) \vdash \wf{C'}\\
   \Delta; \kenv'; \Gamma \vdash \wf{F'}
  }
  {\Delta; (\kenv', a : \poly); \Gamma \vdash \wf{\dec{let}_R\, x =
      \lambda a.\Box \;\dec{in}\; C' :: F'}}
\]
where $\kenv = (\kenv', a : \poly)$
and we have
$f[C] = \Let_R\, x = \letexists{a}C \;\In\; C'$.
%
\js{I'm against using $\poly$ kind when adding things to $\kenv$.  Currently this
  is not defined as part of syntax and I think we don't need an explicit $\poly$
  here.}

By $\{ a \} \uplus \btv(C') \disjoint \btv(F')$ we have $\btv(F) = \{ a \} \uplus \btv(C') \uplus \btv(F')$.
Together with \premissRef{premiss:btv-c-f-disjoint} this gives us
$\btv(f[C]) = \{ a \} \uplus \btv(C') \uplus \btv(C')$
and
$\btv(F') \disjoint \btv(f[C])$ \premissNum{premiss:btv-Fprime-vs-fC}.

We can now derive the following:
\[
\inferrule
  {\btv(C) \disjoint \btv(C')\\
   \Delta; (\kenv', a); \Gamma \vdash \wf{C}\\\\
   \Delta; (\kenv', a); (\Gamma, x : \bot) \vdash \wf{C'}}
  {\Delta; \kenv'; \Gamma \vdash \wf{\Let_{\lbrace \cdot , \mono \rbrace} \; x = \letexists{a} C \;\In\; C'}}
\]

By applying the induction hypothesis
to
$\Delta; \kenv'; \Gamma \vdash \wf{F'}$
and
$\Delta; \kenv'; \Gamma \vdash \wf{f[C]}$ and
\premissRef{premiss:btv-Fprime-vs-fC} we obtain
$\resd{\Delta}{F'}; \resk{\kenv'}{F'}; \resg{\Gamma}{F'} \vdash \wf{F'[f[C]]}$.

We have
$\resd{\Delta}{F}$ = $\resd{\Delta}{F'}$,
$\resk{\kenv}{F}$ = $\resk{\kenv'}{F'}$, and
$\resd{\Gamma}{F}$ = $\resd{\Gamma}{F'}$,
meaning that this is equivalent to the desired property.


\item Case \lab{WF-Stack-DefOut}:

We have a derivation of the form
\[
\inferrule
  {
   \Delta; \kenv \vdash \wf{(\Gamma', x : A)} \\
   \Delta; \kenv; \Gamma' \vdash \wf{F'}}
  {\Delta; \kenv; (\Gamma', x : A) \vdash \wf{\Def\; (x : A) :: F'}}
\]
where $\Gamma = (\Gamma', x : A$).

We can now derive the following:
\[
\inferrule
  {\Delta; \kenv \vdash \wf{(\Gamma', x : A)} \\
   \Delta; \kenv; (\Gamma', x : A) \vdash \wf{C}}
  {\Delta; \kenv; \Gamma' \vdash \wf{\Def\; (x : A) \;\In\; C}}
\]

We have $f[C] = \Def\; (x : A) \;\In\; C$
as well as
$\resd{\Delta}{F}$ = $\resd{\Delta}{F'}$,
$\resk{\kenv}{F}$ = $\resk{\kenv}{F'}$, and
$\resd{\Gamma}{F}$ = $\resd{\Gamma'}{F'}$.

We can obtain
$\btv(F') \disjoint \btv(f[C])$~\premissNum{defout:btv-Fprime-vs-fC}
using the same reasoning as in case \lab{WF-Stack-Forall}.

Applying the induction hypothesis to
$\Delta; \kenv; \Gamma' \vdash \wf{F'}$ and
$\Delta; \kenv; \Gamma' \vdash \wf{f[C]}$ and
\premissRef{defout:btv-Fprime-vs-fC}
then yields the desired property.

\end{itemize}
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../constraint_freezeml"
%%% End:

